GRAM: Graph-based Attention Model for Healthcare Representation Learning

Deep learning methods exhibit promising performance for predictive modeling in healthcare, but two important challenges remain: -Data insufficiency:Often in healthcare predictive modeling, the sample size is insufficient for deep learning methods to achieve satisfactory results. -Interpretation:The representations learned by deep learning methods should align with medical knowledge. To address these challenges, we propose a GRaph-based Attention Model, GRAM that supplements electronic health records (EHR) with hierarchical information inherent to medical ontologies. Based on the data volume and the ontology structure, GRAM represents a medical concept as a combination of its ancestors in the ontology via an attention mechanism. We compared predictive performance (i.e. accuracy, data needs, interpretability) of GRAM to various methods including the recurrent neural network (RNN) in two sequential diagnoses prediction tasks and one heart failure prediction task. Compared to the basic RNN, GRAM achieved 10% higher accuracy for predicting diseases rarely observed in the training data and 3% improved area under the ROC curve for predicting heart failure using an order of magnitude less training data. Additionally, unlike other methods, the medical concept representations learned by GRAM are well aligned with the medical ontology. Finally, GRAM exhibits intuitive attention behaviors by adaptively generalizing to higher level concepts when facing data insufficiency at the lower level concepts.

==> attention_table.tex <==
\begin{table}
\caption{Spearman correlation between a medical code's number of siblings and its attention weight}
\label{tab:spearman}
% \small
\vspace*{-2mm}
\centering
\begin{tabular}{l|c|c|c}
\textbf{Model} & \mname$_{GloVe}$ & \mname & \mname$_{RT}$\\
\hline
\hline
Attention on leaf & 0.48 (0.00e-00) & 0.36 (0.00e-00) & 0.06 (1.17e-10) \\ 
Attention on parent & 0.52 (0.00e-00) & 0.44 (0.00e-00) & -0.04 (1.03e-04)\\
Attention on grandparent & -0.20 (6.15e-87) & 0.06 (1.18e-09) & 0.02 (2.57e-02)\\
Attention on great-grandparent & -0.14 (4.30e-34) & -0.19 (5.62e-63) & 0.03 (5.90e-03)\\
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}

==> hyperparam_table.tex <==
\begin{table}[t]
\caption{Hyper-parameters used by the models in each predictive modeling experiments}
\label{tab:hyperparameter}
% \small
\vspace*{-2mm}
\centering
\begin{footnotesize}
\begin{tabular}{l|l|c|c|c|c|c}
\textbf{Experiment} & \textbf{Model} & $m$ & $r$ & $l$ & $L_2$ & Dropout rate \\ 
\toprule
\multirow{7}{*}{\begin{tabular}{l} Disease progression \\ modeling (Sutter data) \end{tabular}} & \texttt{GRAM}+ & 500 & 500 & 100 & 0.0001 & 0.6 \\ 
& \texttt{GRAM} & 500 & 500 & 100 & 0.0001 & 0.6 \\
& RandomDAG & 500 & 500 & 100 & 0.0001 & 0.6 \\
& RNN+ & 550 & 500 & & 0.0001 & 0.6 \\
& RNN & 550 & 500 & & 0.0001 & 0.6 \\
& SimpleRollUp & 500 & 500 & & 0.0001 & 0.4 \\
& RollUpRare & 500 & 500 & & 0.0001 & 0.2 \\
\midrule
\multirow{7}{*}{\begin{tabular}{l} Disease progression \\ modeling (MIMIC-III) \end{tabular}} & \texttt{GRAM}+ & 400 & 400 & 100 & 0.0001 & 0.6 \\ 
& \texttt{GRAM} & 400 & 400 & 100 & 0.001 & 0.6 \\
& RandomDAG & 400 & 400 & 100 & 0.001 & 0.6 \\
& RNN+ & 550 & 400 & & 0.001 & 0.8 \\
& RNN & 550 & 400 & & 0.001 & 0.8 \\
& SimpleRollUp & 400 & 400 & & 0.001 & 0.6 \\
& RollUpRare & 400 & 400 & & 0.0001 & 0.0 \\
\midrule
\multirow{7}{*}{\begin{tabular}{l} HF prediction \\ (Sutter HF cohort) \end{tabular}} & \texttt{GRAM}+ & 200 & 100 & 100 & 0.001 & 0.6 \\ 
& \texttt{GRAM} & 200 & 100 & 100 & 0.001 & 0.6 \\
& RandomDAG & 300 & 100 & 200 & 0.001 & 0.6 \\
& RNN+ & 200 & 100 & & 0.0001 & 0.6 \\
& RNN & 200 & 100 & & 0.001 & 0.6 \\
& SimpleRollUp & 300 & 200 & & 0.001 & 0.4 \\
& RollUpRare & 100 & 100 & & 0.001 & 0.6 \\
\bottomrule
\end{tabular}
\end{footnotesize}
\vspace{-4.3mm}
\end{table}

==> mimic_dpm_table.tex <==
\begin{table*}
\centering
\small
%\vspace*{-2mm}
\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0086}&\textbf{0.1089}&\textbf{0.1665}&0.1029&0.2597\\
GRAM&0.0000&0.0468&0.1093&0.0918&\textbf{0.2665}\\
RandomDAG&0.0000&0.0327&0.0778&0.0612&0.1634\\
RNN+&0.0000&0.0435&0.1266&0.0973&0.2594\\
RNN&0.0000&0.0376&0.1105&0.0923&0.2601\\
SimpleRollUp&0.0000&0.0671&0.1501&\textbf{0.1191}&0.2635\\
RollUpRare&0.0000&0.0423&0.1085&0.0874&0.2604\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@5} of sequential diagnoses prediction on MIMIC-III}
\label{tab:sdp_mimic_5}
\end{subtable}

\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0380}&\textbf{0.1310}&\textbf{0.2095}&0.1627&0.4175\\
GRAM&0.0045&0.0682&0.1494&0.1487&0.4235\\
RandomDAG&0.0023&0.0470&0.1025&0.0938&0.2692\\
RNN+&0.0227&0.0587&0.1591&0.1616&0.4193\\
RNN&0.0023&0.0518&0.1389&0.1521&0.4142\\
SimpleRollUp&0.0249&0.1038&0.1997&\textbf{0.1769}&\textbf{0.4260}\\
RollUpRare&0.0227&0.0530&0.1412&0.1519&0.4180\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@10} of sequential diagnoses prediction on MIMIC-III}
\label{tab:sdp_mimic_10}
\end{subtable}

\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0672}&\textbf{0.1787}&\textbf{0.2644}&0.2490&0.6267\\
GRAM&0.0556&0.1016&0.1935&0.2296&0.6363\\
RandomDAG&0.0329&0.0708&0.1346&0.1512&0.4494\\
RNN+&0.0454&0.0843&0.2080&0.2494&0.6239\\
RNN&0.0454&0.0731&0.1804&0.2371&0.6243\\
SimpleRollUp&0.0578&0.1328&0.2455&\textbf{0.2667}&\textbf{0.6387}\\
RollUpRare&0.0454&0.0653&0.1843&0.2364&0.6277\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@20} of sequential diagnoses prediction on MIMIC-III}
\label{tab:sdp_mimic_20}
\end{subtable}

\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0744}&\textbf{0.2065}&\textbf{0.3180}&0.3363&0.7726\\
GRAM&0.0578&0.1157&0.2257&0.3074&\textbf{0.7802}\\
RandomDAG&0.0351&0.0932&0.1635&0.2200&0.5977\\
RNN+&0.0578&0.1103&0.2571&0.3409&0.7656\\
RNN&0.0578&0.0775&0.2237&0.3160&0.7643\\
SimpleRollUp&0.0578&0.1556&0.2865&\textbf{0.3488}&0.7800\\
RollUpRare&0.0556&0.0910&0.2235&0.3255&0.7661\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@30} of sequential diagnoses prediction on MIMIC-III}
\label{tab:sdp_mimic_30}
\end{subtable}

\caption{Accuracy at various $k$'s (a to d) for sequential diagnoses prediction on MIMIC-III. The columns represent the labels grouped by the percentile of their frequencies in the training data in non-decreasing order.}
\label{tab:mimic_dpm}
\end{table*}

==> old_attention_figures.tex <==
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figs/dpm_leaf_attention}
  \caption{Attention weights on the leaf nodes when performing DPM on Sutter data.}
  \label{fig:leaf_attention}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figs/dpm_parent_attention}
  \caption{Attention weights on the parent nodes when performing DPM on Sutter data.}
  \label{fig:parent_attention}
\end{subfigure}

\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figs/hf_leaf_attention}
  \caption{Attention weights on the leaf nodes when performing HF prediction on Sutter HF cohort.}
  \label{fig:leaf_attention}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figs/hf_parent_attention}
  \caption{A subfigure}
  \label{fig:leaf_attention}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:attention}
\end{figure}

==> old_exp.tex <==
We show that \mname can improve the performance when faced with data insufficiency by learning accurate and interpretable representations of medical concepts. We first describe experiment setup, then report the predictive performance of \mname with various baseline models in terms of disease progression modeling and heart failure (HF) prediction. After discussing \mname's scalability, we qualitatively evaluate the interpretability of the resulting representation.  
The source code of \mname is publicly available at \url{https://github.com/mp2893/gram}.

\subsection{Experiment Setup}
\input{data_stat.tex}
\textbf{Source of data:} We use three real EHR datasets to evaluate \mname: 1)  Sutter Palo Alto Medical Foundation (PAMF) dataset consists of medical records of 258K patients over 18 years; 2) MIMIC-III dataset \citep{johnson2016mimic, goldberger2000physiobank} consist of medical records of 7.5K intensive care unit (ICU) patients over 11 years; 
3) Sutter heart failure (HF) cohort which was a subset of PAMF data for a heart failure onset prediction study with  3.4K HF cases and 27K controls chosen by a set of criteria (see Appendix \ref{appendix:cohort}). 
We extracted ICD9 diagnosis codes from its encounter records. A summary of the datasets are provided in Table~\ref{tab:data_stats}. 
% \jimeng{why don't we use other sources such as medication and procedure? It seems we can also include those sources as well which may improve the prediction accuracy further.}
% Using additional information such as medication orders or procedure orders can increase predictive performance, but in this paper we focus on comparing how \mname and other baselines perform under data insufficiency.

\textbf{Implementation details:} We implemented \mname with Theano 0.8.2 \citep{team2016theano}. For training models, we used Adadelta \citep{zeiler2012adadelta} with a mini-batch of 100 patients, on a machine equipped with Intel Xeon E5-2640, 256GB RAM, four Nvidia Titan X's and CUDA 7.5. 
\newline
We used CCS multi-level diagnoses hierarchy\footnote{https://www.hcup-us.ahrq.gov/toolssoftware/ccs/AppendixCMultiDX.txt} as our knowledge DAG $\mathcal{G}$. We also tested the ICD9 code hierarchy\footnote{http://www.icd9data.com/2015/Volume1/default.htm}, but the performance was similar to using CCS multi-level hierarchy. %We left using SNOMED-CT for future work because it uses its own diagnosis codes, which have $m$-to-$n$ mapping relations with ICD9 diagnosis codes.

\textbf{Prediction tasks:} We performed disease progression modeling on Sutter data and MIMIC-III. We also performed HF onset prediction on Sutter HF cohort.
\newline
\textit{Disease progression modeling} aims at predicting all the diagnosis categories in the next visit. In this case we prepared the true labels $\yb_{t}$ by grouping the ICD9 codes into 283 groups by using CCS single-level diagnosis grouper\footnote{https://www.hcup-us.ahrq.gov/toolssoftware/ccs/AppendixASingleDX.txt}. 
This is to improve the training speed and predictive performance for easier analysis, while preserving sufficient granularity for each diagnosis.
\newline
\textit{HF onset prediction} is a binary prediction task for the new HF diagnosis. The prediction is made only once at the last visit $\xb_T$.%, using the sigmoid function instead of the Softmax function. 
\newline
For both prediction tasks, we randomly divide the dataset into the training, validation and test set by 0.75:0.10:0.15 ratio, and use the validation set to tune the hyper-parameters. Further details regarding the hyper-parameter tuning are provided in Appendix \ref{appendix:hyperparameter}.

\textbf{Models:} We compare the following models where the first two  {\texttt{GRAM}+} and {\texttt{GRAM}} are the proposed methods and the rest are baselines. Hyper-parameter tuning is configured so that the baselines' number of parameters would be comparable to \texttt{GRAM}'s. Further details are provided in Appendix \ref{appendix:hyperparameter}.
\begin{itemize}[leftmargin=5.5mm]
\item
\textbf{\mname:} Input sequence $\xb_1, \ldots, \xb_T$ is first transformed by the embedding matrix $\Gb$, then fed to the GRU with a single hidden layer, which in turn makes the prediction, as described by Eq.\eqref{eq:rnn_prediction}. The basic embeddings $\eb_i$'s are randomly initialized.
\item
\textbf{\texttt{GRAM}+:} We use the same setup as \textbf{\texttt{GRAM}+}, but the basic embeddings $\eb_i$'s are initialized with GloVe vectors trained with the co-occurrence ofover all leaf and internal concepts of the knowledge DAG (see Section \ref{sec:emb}).
\item
\textbf{RandomDAG:} We use the same setup as \textbf{\mname}, but we use a knowledge DAG where all leaves have five randomly assigned ancestors from the CCS multi-level hierarchy. This is to test the effect of correct domain knowledge as opposed to simply increasing the number of model parameters.
\item
\textbf{RNN}: Input $\xb_t$ is transformed by an embedding matrix $\Wb_{emb} \in \mathbb{R}^{k \times |\mathcal{C}|}$, then fed to the GRU with a single hidden layer. The embedding size $k$ is a hyper-parameter. $\Wb_{emb}$ is randomly initialized and trained together with the GRU.
\item
\textbf{RNN+:} We use the same setup as \textbf{RNN}, but we initialize the embedding matrix $\Wb_{emb}$ with GloVe vectors trained only with the co-occurrence of leaf concepts. This is to compare \mname with a similar weight initialization technique.
\item
\textbf{SimpleRollUp:} We use the same setup as \textbf{RNN}. But for input $\xb_t$, we replace all diagnosis codes with their direct parent codes in the CCS multi-level hierarchy, giving us 578, 526 and 517 input codes respectively for Sutter data, MIMIC-III and Sutter HF cohort. This is to compare the performance of \mname with a common grouping technique.  
\item
\textbf{RollUpRare:} We use the same setup as \textbf{RNN}, but we replace any diagnosis code whose frequency is less than a certain threshold in the dataset with its direct parent. We set the threshold to 100 for Sutter data and Sutter HF cohort, and 10 for MIMIC-III, giving us 4,408, 935 and 1,538 input codes respectively for Sutter data, MIMIC-III and Sutter HF cohort. This is an intuitive way of dealing with infrequent medical codes.
\end{itemize}

\subsection{Prediction performance and scalability}
\label{ssec:exp_prediction}
\input{exp_prediction.tex}

%\subsection{\ecedit{Scalability of \mname}}
%\label{ssec:exp_scalability}
\input{exp_scalability.tex}

\subsection{Qualitative evaluation of interpretable representations}
\label{ssec:exp_tsne}
\input{exp_tsne.tex}

\subsection{Analysis of the attention behavior}
\label{ssec:exp_attention}
\input{exp_attention.tex}

==> old_exp_attention.tex <==
%\begin{figure}[t]
%\caption{Each row respectively shows the attention behavior in DPM for Sutter data and HF prediction for Sutter HF cohort. First two columns respectively show the attention weight on the diseases (\textit{e.g.} leaf nodes) and their direct parents, averaged by the percentile of the disease's frequency in the training data in non-decreasing order. Last two columns are the same, but the X-axis is the percentile of each disease's number of siblings. In each plot, we show Spearman correlation and the p-value in the parenthesis.}
%\centering
%\label{fig:attention_all}
%\includegraphics[width=\textwidth]%{./Figs/attentions_all}
%\end{figure}

In this subsection, we study the attention behavior of \mname in two different tasks: DPM on Sutter data and HF prediction on Sutter HF cohort. For both prediction tasks we calculate for each disease the attention weight on itself and its direct parent using Eq.\eqref{eq:attention_function} and Eq.\eqref{eq:softmax}. Then we sort the results by each disease's number of occurrences in the training data in non-decreasing order to plot Figures \ref{fig:attention_all}a, b, e and f. We also sort the results by each disease's number of siblings in the CCS multi-level tree in non-decreasing order to plot Figures \ref{fig:attention_all}c, d, g and h. Note that Figures \ref{fig:attention_all}a, b, c, and d are for DPM on Sutter data and Figures \ref{fig:attention_all}e, f, g and h are for HF prediction on Sutter HF cohort.

Figures \ref{fig:attention_all}a and b show that for DPM, the disease frequency does not have a clear relationship with the amount of attention being paid to either the disease itself or its parent. Figures \ref{fig:attention_all}c, however, tells us that more siblings a disease has, more attention it receives\footnote{Quite the contrary to reality.}. This makes sense because a parent with many children tends to hold more abstract information than a parent with few children. Therefore you should pay more attention to the children, the disease itself, lest you should lose fine-grained information. Figure \ref{fig:attention_all}d tells us that a parent with many children also receives more attention  than a parent with few children. This again is logical because where there is more information, the more attention we should pay. 

Interestingly, Figures \ref{fig:attention_all}e and f tell us that, for HF prediction, disease frequency plays a significant role in the attention mechanism. Figure \ref{fig:attention_all}e says that the more you observe a disease, the more attention it receives. Figure \ref{fig:attention_all}f, on the other hand, says that the more you observe a disease, the less attention is given to its parent. This is very logical because as you observe a certain disease many times, you become more confident about your knowledge of it. In the same spirit, the more confident you are about a certain disease, you become less dependent on its parent. This behavior is clearly illustrated by the opposite correlation values in Figures \ref{fig:attention_all}e and f. Figures \ref{fig:attention_all}g and h are showing similar behaviors to Figures \ref{fig:attention_all}c and d, which is logical, so we will not reiterate the same logic.

Now we turn to the different behavior shown by Figures \ref{fig:attention_all}a, b and Figures \ref{fig:attention_all}e, f. Why does disease frequency affect the attention mechanism in HF prediction but not in DPM? This can be explained by the absolute amount of attention paid to the leaf nodes (\textit{e.g.} diseases). Figures \ref{fig:attention_all}a and c shows that the amount of attention paid to the leaf nodes is at least three orders of magnitude smaller than what is paid to the parent nodes. However, in HF prediction, the amounts of attention paid to both leaf nodes and parent nodes are in the same order of magnitude. This means that the leaf nodes play a minimal role in DPM, and therefore their frequencies do not really matter to the attention mechanism. HF prediction, on the other hand, requires the information provided by the leaf nodes, and therefore their frequencies have an impact to the attention mechanism. 

This is exactly why RNN$_G$ was the best baseline for DPM but not for HF prediction. Since DPM is not very dependent on the leaf node information, simply replacing all disease codes with their direct parents was sufficient to obtain competitive performance. HF prediction, however, heavily utilizes the leaf node information and that makes RNN$_G$ less competitive than RNN$_{+}$. We believe the reason why DPM is not very dependent on the leaf node information is that we group the output labels with CCS single-level disease grouper that groups the entire disease codes into 283 categories. Since the complexity of the output labels is significantly reduced, using 578 parent codes instead of 10,437 disease codes as input seems enough to achieve competitive performance.

==> setting.tex <==
\usepackage{bm,amsmath,amssymb}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{longtable,lscape}
\usepackage[normalem]{ulem}
\usepackage{booktabs}
\usepackage{xspace}
\usepackage{natbib}
\RequirePackage{color}
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\hypersetup{ % play with the different link colors here
    colorlinks,
    citecolor=mydarkblue,
    filecolor=mydarkblue,
    linkcolor=mydarkblue,
    urlcolor=mydarkblue % set to black to prevent printing blue links
}
% \usepackage[sort, numbers]{natbib}
\usepackage{subcaption}
\usepackage{multirow}
% \usepackage{wrapfig}
%\usepackage{floatrow}
%\floatsetup[table]{capposition=top}
\usepackage{url}
\newcommand{\tbedit}[1]{\textcolor{magenta}{\emph{[TB: #1]}}}
\newcommand{\jsedit}[1]{\textcolor{green}{\emph{[JS: #1]}}}
\newcommand{\ecedit}[1]{\textcolor{blue}{\emph{[EC: #1]}}}
\newcommand{\blue}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\mname}{\texttt{GRAM}\xspace}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
% \usepackage[top=1in, bottom=1.25in, left=1in, right=1in]{geometry}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{enumitem}
\usepackage{threeparttable}
\usepackage{bm}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

==> sutter_dpm_table.tex <==
\begin{table*}
\centering
\small
%\vspace*{-2mm}
\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0150}&\textbf{0.3242}&0.4325&0.4238&0.4903\\
GRAM&0.0042&0.2987&0.4224&0.4193&0.4895\\
RandomDAG&0.0050&0.2700&0.4010&0.4059&0.4853\\
RNN+&0.0069&0.2742&0.4140&0.4212&\textbf{0.4959}\\
RNN&0.0080&0.2691&0.4134&0.4227&0.4951\\
SimpleRollUp&0.0085&0.3078&\textbf{0.4369}&\textbf{0.4330}&0.4924\\
RollUpRare&0.0062&0.2768&0.4176&0.4226&0.4956\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@5} of sequential diagnoses prediction on Sutter data}
\label{tab:sdp_sutter_5}
\end{subtable}

\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0319}&\textbf{0.3882}&0.5054&0.5215&0.6459\\
GRAM&0.0163&0.3645&0.4944&0.5173&0.6445\\
RandomDAG&0.0142&0.3285&0.4691&0.5025&0.6401\\
RNN+&0.0183&0.3412&0.4884&0.5233&\textbf{0.6538}\\
RNN&0.0196&0.3290&0.4871&0.5230&0.6531\\
SimpleRollUp&0.0164&0.3768&\textbf{0.5132}&\textbf{0.5326}&0.6521\\
RollUpRare&0.0204&0.3450&0.4917&0.5228&0.6535\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@10} of sequential diagnoses prediction on Sutter data}
\label{tab:sdp_sutter_10}
\end{subtable}

\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0630}&0.4486&0.5764&0.6153&0.7973\\
GRAM&0.0442&0.4276&0.5669&0.6125&0.7963\\
RandomDAG&0.0397&0.3933&0.5389&0.5997&0.7919\\
RNN+&0.0483&0.4132&0.5654&0.6235&0.8003\\
RNN&0.0481&0.4025&0.5630&0.6232&0.7995\\
SimpleRollUp&0.0418&\textbf{0.4496}&\textbf{0.5877}&\textbf{0.6262}&\textbf{0.8013}\\
RollUpRare&0.0517&0.4170&0.5672&0.6214&0.8002\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@20} of sequential diagnoses prediction on Sutter data}
\label{tab:sdp_sutter_20}
\end{subtable}

\begin{subtable}{1.\textwidth}
\centering
\begin{tabular}{l|c|c|c|c|c}
Model & 0-20 & 20-40 & 40-60 & 60-80 & 80-100\\ 
\toprule
GRAM+&\textbf{0.0946}&0.4879&0.6186&0.6792&\textbf{0.8800}\\
GRAM&0.0662&0.4693&0.6107&0.6766&0.8798\\
RandomDAG&0.0672&0.4313&0.5843&0.6667&0.8760\\
RNN+&0.0736&0.4604&0.6136&\textbf{0.6930}&0.8785\\
RNN&0.0733&0.4478&0.6103&0.6921&0.8767\\
SimpleRollUp&0.0662&\textbf{0.4924}&\textbf{0.6312}&0.6907&0.8795\\
RollUpRare&0.0759&0.4657&0.6146&0.6908&0.8778\\
\bottomrule
\end{tabular}
\caption{\textit{Accuracy@30} of sequential diagnoses prediction on Sutter data}
\label{tab:sdp_sutter_30}
\end{subtable}

\caption{Accuracy at various $k$'s (a to d) for sequential diagnoses prediction on Sutter data. The columns represent the labels grouped by the percentile of their frequencies in the training data in non-decreasing order.}
\label{tab:sutter_dpm}
\end{table*}
